Surround-view Fisheye Camera Perception for Automated Driving: Overview, Survey and Challenges

Surround-view fisheye cameras are commonly used for near-field sensing in automated driving. Four fisheye cameras on four sides of the vehicle are sufficient to cover 360{\deg} around the vehicle capturing the entire near-field region. Some primary use cases are automated parking, traffic jam assist, and urban driving. There are limited datasets and very little work on near-field perception tasks as the focus in automotive perception is on far-field perception. In contrast to far-field, surround-view perception poses additional challenges due to high precision object detection requirements of 10cm and partial visibility of objects. Due to the large radial distortion of fisheye cameras, standard algorithms cannot be extended easily to the surround-view use case. Thus, we are motivated to provide a self-contained reference for automotive fisheye camera perception for researchers and practitioners. Firstly, we provide a unified and taxonomic treatment of commonly used fisheye camera models. Secondly, we discuss various perception tasks and existing literature. Finally, we discuss the challenges and future direction.

==> include/biographies.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,clip,keepaspectratio]{images/bio/varun.jpg}}]{Varun Ravi Kumar} received a Ph.D. degree in Artificial Intelligence from TU Ilmenau in 2021 and an M.Sc. degree in 2017 from TU Chemnitz, Germany. Ph.D. thesis builds a first-ever 6-task multi-task learning near-field perception system that constitutes the necessary modules for a Level3 autonomous stack using surround-view fisheye cameras. His research mainly focuses on designing self-supervised perception algorithms using neural networks for self-driving cars. His diverse expertise lies in geometric, semantic tasks, 2D \& 3D object detection, point-cloud processing \& multi-task modeling. He was awarded the \textit{Deutschlandstipendium} for top-class international talent. He has 23 publications and two patents in top robotics and vision conferences.
\end{IEEEbiography}
\vskip 0pt plus -1fil
% -------------------------------------------------
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/ciaran}}]
{Ciar\'{a}n Eising} obtained his Ph.D. in Computer Engineering at NUI Galway in 2010. From 2009 to 2020, Ciar\' {a}n was a computer vision architect and Senior Expert in Valeo Ireland. In 2020, Ciar\'{a}n joined the University of Limerick as a lecturer in Computer Vision and Artifical Intelligence.
\end{IEEEbiography}
\vskip 0pt plus -1fil
% -------------------------------------------------
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/ciaran}}]
{Christian Witt}  is an \sy{add bio and pic}
obtained his Master in Physics at the Technical University of Dresden in 2017. Since 2017 he is working in Driving Assistance Research at Valeo, where he also held the title of Expert. Since 2021, Christian is team lead for data recording and tooling.
In reality, he does not look like Ciar\'{a}n, but was just too lazy to upload a picture. 
\cw{not much to tell to be honest}
\end{IEEEbiography}
% -------------------------------------------------
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/senthil1}}]{Senthil Yogamani}
is an Artificial Intelligence architect and holds a director level technical leader position at Valeo Ireland. He leads the research and design of AI algorithms for various modules of autonomous driving systems. He has over 17 years of experience in computer vision and machine learning including 14 years of experience in industrial automotive systems. He is an author of 100+ publications with 3000+ citations and 100+ inventions with 75 filed patent families. He serves on the editorial board of various leading IEEE automotive conferences including ITSC and IV and advisory board of various industry consortia including Khronos, Cognitive Vehicles and IS Auto. He is a recipient of the best associate editor award at ITSC 2015 and best paper award at ITST 2012.
\end{IEEEbiography}
\vskip 0pt plus -1fil
% -------------------------------------------------
